Learning in Online Principal-Agent Interactions: The Power of Menus

We study a ubiquitous learning challenge in online principal-agent problems during which the principal learns the agent's private information from the agent's revealed preferences in historical interactions. This paradigm includes important special cases such as pricing and contract design, which have been widely studied in recent literature. However, existing work considers the case where the principal can only choose a single strategy at every round to interact with the agent and then observe the agent's revealed preference through their actions. In this paper, we extend this line of study to allow the principal to offer a menu of strategies to the agent and learn additionally from observing the agent's selection from the menu. We provide a thorough investigation of several online principal-agent problem settings and characterize their sample complexities, accompanied by the corresponding algorithms we have developed. We instantiate this paradigm to several important design problems $-$ including Stackelberg (security) games, contract design, and information design. Finally, we also explore the connection between our findings and existing results about online learning in Stackelberg games, and we offer a solution that can overcome a key hard instance of Peng et al. (2019).

==> related.tex <==
%\subsection{Related Work}\label{sec:related}
%There are several lines of research that are most relevant to ours. 
%First, repeated games in auctions, a.k.a dynamic pricing, is an emerging area of interest \cite{den2015dynamic}, but there is a rich history of research on this repeated setting in the absence of realistic assumption on buyer's behavior. Starting from \cite{kleinberg2003value}, Kleinberg and Leighton studied the regret of a repeated posted price auction where a seller selling unlimited supply of some identical goods to buyers with three valuation models. Amin et al. \cite{amin2015online} study the problem from a different perspective, revenue maximization in repeated posted price auctions, where a seller iteratively interacts with a single buyer whose has a linear utility model. \cite{roth2016watch} studied a related problem of optimizing seller's revenue via interacting with a fixed buyer whose valuations function is not limited to be linear but concave. Roth et al. also extended the setting of \cite{roth2016watch} from fixed buyer valuation to a stochastic setting where buyer's valuation is drawn from an unknown distribution \cite{roth2020multidimensional}. However, all of these previous works assume that buyers act truthfully according to their private valuation model. 
%
%On the other hand, Amin et al. \cite{amin2013learning, amin2014repeated} proposed the regret minimization algorithms for the seller against \textit{strategic} buyers in repeated posted price auctions (see also \cite{drutsa2017horizon,drutsa2018weakly,mohri2014optimal,mohri2015revenue}). Compared to regret minimization, the literature on revenue optimization in repeated posted price auctions with strategic buyers is still understudied.  Devanur et al. studied the Fishmonger problem \cite{devanur2014perfect} where a single seller sells a single item to a single buyer for $T$ rounds, and the buyer's value of the item is drawn from some distribution. A very recent literature studied the problem of expected cumulative revenue optimization for repeated posted-price auctions where a seller interacts with a single buyer \cite{vanunts2019optimal} and the seller and the buyer have different discounting factors over their expected utilities in the future. 
%
%A distinguishing characteristic of our model is we consider the objective of the strategic buyer instead of standing from the seller's perspective like all the previous work does. We study the optimal strategic behavior of the buyer so that they can optimize their utility  against any seller with effective learning strategy. In addition, we want to emphasize that although our model involves dynamic interactions between the seller and the buyer like repeated games, we don't care about the cumulative utility achieved by the buyer and seller. We study the utility the seller and buyer can achieve at the equilibrium of the game, so our model can also be thought as a single-shot valuation model reporting game in which the buyer strategically reports his valuation model and the seller best-responds accordingly.
%
%Second, our problem can also be viewed as an instance of Stackelberg game problem \cite{roth2016watch,gan2019imitative}, a well-studied game model in which the leader (seller) first commits to an action and follower (buyer) plays his best response after observing the leader's action. There is a large literature on strategic behavior analysis in Stackelberg games \cite{yin2013optimal,xu2015exploring,schlenker2018deceiving}, but all of them focus on the leader's strategic analysis. 
%On the other hand, the buyer's strategic behavior is still understudied. A recent literature studied leader's learning algorithms against strategic follower in general Stackelberg games and Stackelberg security games \cite{gan2019manipulating,gan2019imitative}. Our game model can be thought as a specific Stackelberg pricing game which is different from their work. Deng \cite{deng2019strategizing} et al. studied a related problem of strategic leader against no-regret learner. Braverman et al. also study the interaction between the strategic leader and the no-regret learner under the pricing game condition \cite{braverman2018selling}. Their work stands from the seller's view and study how to sell the item to a no-regret buyer. Our problem can also be thought as a specific version of Deng et al's work under the pricing game setting. Unlike Braverman et al.'s work, we consider a reverse Stackelberg game where the buyer is the leader because the seller has no information about the buyer‘s valuation, and the buyer can choose what kind of valuation information to report and thus influence the pricing strategy offered by the seller. In addition, our work differs from Deng et al's work in two ways. On the one hand, our learner (seller) is not limited to no-regret learning algorithms, they can use any effective learning strategy. On the other hand, we provide a specific characterization of the strategic behavior model for the buyer while they didn't. Nedelec et al. \cite{nedelec2018bidder,nedelec2019adversarial,nedelec2019learning} study the optimal bidding strategy of the buyer in revenue-maximizing auctions where the buyer optimize their long-term expected utility through some machine learning techniques. More related to our article is Tang and Zeng \cite{tang2018price} who study the problem of committing to a fake type distribution and acts rationally as if the follower's type were from the fake type distribution. The primary novel contribution of our work, compared to this body of literature, is two-fold. First, we have production cost but the auction setting does not have production cost. If there is no production cost, then optimal deception is trivial, i.e., pretending to have valuation function of 0. This recovers the result of \cite{tang2018price} when restricted to a single bidder. Second, we consider the setup with multiple items for sell while a significant part of the literature only considers single-item auctions \cite{amin2013learning,amin2014repeated,mohri2014optimal,mohri2015revenue,vanunts2019optimal,tang2018price}.
%
%Finally, our work is also closely related to the classic revealed preference problems in which the buyer has a fixed but unknown utility function \cite{varian2006revealed}. This problem was first proposed by Samuelson \cite{samuelson1938note}, and \cite{mas1995microeconomic,rubinstein2012lecture} provide some textbook introduction to the model. In this line of work, the goal is to find the buyer's utility function. Afrait proposed a fundamental theorem which shows how to construct a utility function to match the sequence of observations and under what condition this construction is possible \cite{afriat1967construction}, but the constructed utility function is too specific to the revealed preferences and doesn't generalize well on future observations. Beigman and Vohra proposed to use a \textit{probably approximately correct} (PAC) method to learn the utility function such that it also predicts well on future preferences revealed by the buyer \cite{beigman2006learning}.
%
%%\hf{For those that are very closed related to ours, need to elaborate the major difference between their work and ours }

\subsection{Related Work}\label{sec:related}
There are several lines of research that are most relevant to ours. 
First, repeated games in auctions, a.k.a dynamic pricing, is an emerging area of interest \cite{den2015dynamic}, but there is a rich history of research on this repeated setting in the absence of realistic assumption on buyer's behavior. Starting from \cite{kleinberg2003value}, Kleinberg and Leighton studied the regret of a repeated posted price auction where a seller selling unlimited supply of some identical goods to buyers with three different valuation models. Amin et al. \cite{amin2015online} study the problem from a different perspective, revenue maximization in repeated posted price auctions, where a seller repeatedly interacts with a single buyer who has a linear utility model. \cite{roth2016watch} studied a related problem of optimizing seller's revenue via interacting with a fixed buyer whose valuations function is not limited to be linear but concave. Roth et al. also extended the setting of \cite{roth2016watch} from fixed buyer valuation to a stochastic setting where buyer's valuation is drawn from an unknown distribution \cite{roth2020multidimensional}. However, all of these previous works assume that buyers act truthfully according to their private valuation model. 

On the other hand, Amin et al. \cite{amin2013learning, amin2014repeated} proposed the regret minimization algorithms for the seller against \textit{strategic} buyers in repeated posted price auctions (see also \cite{drutsa2017horizon,drutsa2018weakly,mohri2014optimal,mohri2015revenue}). But the literature on revenue optimization in repeated posted price auctions with strategic buyers is still understudied.  Devanur et al. studied the equilibria of Fishmonger problem \cite{devanur2014perfect} where a single seller sells a single item to a single buyer for $T$ rounds and showed the power of commitment to prices from the seller's point of view. A very recent literature studied the problem of expected cumulative revenue optimization for repeated posted-price auctions where a seller interacts with a single buyer \cite{vanunts2019optimal} and the seller and the buyer have different discounting factors over their expected utilities in the future. 

A distinguishing characteristic of our model is we consider the objective of the strategic buyer instead of standing from the seller's perspective like all the previous work does. We study the optimal strategic behavior of the buyer so that they can optimize their utility  against any seller with effective learning strategy. In addition, we want to emphasize that although our model involves dynamic interactions between the seller and the buyer like repeated games, we don't care about the cumulative utility achieved by the buyer and seller during the learning process. We study the utility achieved by the seller and buyer at the steady stage resulted from a converged sequence of interactions where both agents don't need to update their actions anymore, so our model can also be thought as a single-shot valuation model reporting game in which the buyer strategically reports his valuation model and the seller best-responds accordingly.

Second, our problem can also be viewed as an instance of Stackelberg game problem \cite{roth2016watch,gan2019imitative}, a well-studied game model in which the leader (seller) first commits to an action and follower (buyer) plays his best response after observing the leader's action. There is a large literature on strategic behavior analysis in Stackelberg games \cite{yin2013optimal,xu2015exploring,schlenker2018deceiving}, but all of them focus on the leader's strategic analysis. 
On the other hand, the buyer's strategic behavior is still understudied. A recent literature studied leader's learning algorithms against strategic follower in general Stackelberg games and Stackelberg security games \cite{gan2019manipulating,gan2019imitative}. Our game model can be thought as a specific Stackelberg pricing game which is different from their work. Deng \cite{deng2019strategizing} et al. studied a related problem of strategic leader against no-regret learner. Braverman et al. also study the interaction between the strategic leader and the no-regret learner under the pricing game condition \cite{braverman2018selling}. Their work stands from the seller's view and study how to sell the item to a no-regret buyer. Our problem can also be thought as a specific version of Deng et al's work under the pricing game setting. Unlike Braverman et al.'s work, we consider a reverse Stackelberg game where the buyer is the leader because the seller has no information about the buyer‘s valuation, and the buyer can choose what kind of valuation information to report and thus influence the pricing strategy offered by the seller. In addition, our work differs from Deng et al's work in two ways. On the one hand, our learner (seller) is not limited to no-regret learning algorithms, they can use any effective learning strategy. On the other hand, we provide a specific characterization of the strategic behavior model for the buyer while they didn't. Nedelec et al. \cite{nedelec2018bidder,nedelec2019adversarial,nedelec2019learning} study the optimal bidding strategy of the buyer in revenue-maximizing auctions where the buyer optimize their long-term expected utility through some machine learning techniques. More related to our article is Tang and Zeng \cite{tang2018price} who study the problem of committing to a fake type distribution and acts rationally as if the follower's type were from the fake type distribution. The primary novel contribution of our work, compared to this body of literature, is two-fold. First, we have production cost but the auction setting does not have production cost. Production cost is important. With production cost of 0, the optimal manipulation is trivial, i.e. the buyer pretends to have a value function of 0 to induce a final price of 0 from the seller. The seller is still willing to produce the product even if the price is 0 because it costs her nothing to produce. Second, we consider the setup with multiple items for sell while a significant part of the literature only considers single-item auctions \cite{amin2013learning,amin2014repeated,mohri2014optimal,mohri2015revenue,vanunts2019optimal,tang2018price}. 

Finally, our work is also closely related to the classic revealed preference problems in which the buyer has a fixed but unknown utility function \cite{varian2006revealed}. This problem was first proposed by Samuelson \cite{samuelson1938note}, and \cite{mas1995microeconomic,rubinstein2012lecture} provide some textbook introduction to the model. In this line of work, the goal is to find the buyer's utility function. Afrait proposed a fundamental theorem which shows how to construct a utility function to match the sequence of observations and under what condition this construction is possible \cite{afriat1967construction}, but the constructed utility function is too specific to the revealed preferences and doesn't generalize well on future observations. Beigman and Vohra proposed to use a \textit{probably approximately correct} (PAC) method to learn the utility function such that it also predicts well on future preferences revealed by the buyer \cite{beigman2006learning} and they show that we need conditions which are stricter than the condition proposed by Afrait to compute utility functions that can also predict well on future observations.  Zadimoghaddam and Roth study revealed preferences from the buyer with some specific utility functions and provide efficient algorithms to learn the buyer's utility function which is consistent with revealed preferences and can also predict well on future revealed preferences \cite{zadimoghaddam2012efficiently}. In  \cite{amin2015online}, the authors study revealed preferences from a different perspective, in which the goal is not to learn the buyer's utility function but to achieve profit maximization. However, all these previous works assume that the buyer reveal their preferences honestly which might not be true in practice. Our primary contribution, relative to this line of work, is that we allow manipulation behavior from the buyer. Similar to our work, Cummings et al. also study the revealed preference problem assuming the buyer is strategic \cite{cummings2016empirical}. They prove that little can be inferred about buyer's preferences when the buyer is strategic which is complementary to our work.

